Multi-Order Networks for Action Unit Detection

Action Units (AU) are muscular activations used to describe facial expressions. Therefore accurate AU recognition unlocks unbiaised face representation which can improve face-based affective computing applications. From a learning standpoint AU detection is a multi-task problem with strong inter-task dependencies. To solve such problem, most approaches either rely on weight sharing, or add explicit dependency modelling by decomposing the joint task distribution using Bayes chain rule. If the latter strategy yields comprehensive inter-task relationships modelling, it requires imposing an arbitrary order into an unordered task set. Crucially, this ordering choice has been identified as a source of performance variations. In this paper, we present Multi-Order Network (MONET), a multi-task method with joint task order optimization. MONET uses a differentiable order selection to jointly learn task-wise modules with their optimal chaining order. Furthermore, we introduce warmup and order dropout to enhance order selection by encouraging order exploration. Experimentally, we first demonstrate MONET capacity to retrieve the optimal order in a toy environment. Second, we validate MONET architecture by showing that MONET outperforms existing multi-task baselines on multiple attribute detection problems chosen for their wide range of dependency settings. More importantly, we demonstrate that MONET significantly extends state-of-the-art performance in AU detection.

==> figures/toy/exploration_export.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}
\definecolor{color4}{rgb}{0.505882352941176,0.447058823529412,0.701960784313725}

\begin{axis}[
legend cell align={right},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.66,0.56)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epochs},
xmin=38.5, xmax=511.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy},
ymin=0.76419198602438, ymax=0.969408004581928,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
60 0.773519986867905
70 0.787399992346764
80 0.800359997153282
90 0.809839987754822
100 0.816000002622604
110 0.823240000009537
120 0.831279999017715
130 0.835920003056526
140 0.845039966702461
150 0.852359998226166
160 0.860760006308556
170 0.866799995303154
180 0.87163999080658
190 0.875879988074303
200 0.878600001335144
210 0.881079992651939
220 0.882319983839989
230 0.887879997491837
240 0.889079988002777
250 0.887599992752075
260 0.893200007081032
270 0.894879990816116
280 0.895759990811348
290 0.900959998369217
300 0.902080011367798
310 0.905720010399818
320 0.908360001444817
330 0.907999992370605
340 0.908079978823662
350 0.912440013885498
360 0.913519996404648
370 0.917640009522438
380 0.918239983916283
390 0.91895999610424
400 0.921879979968071
410 0.923160004615784
420 0.924679991602898
430 0.927039995789528
440 0.929519999027252
450 0.927959984540939
460 0.930719992518425
470 0.930439999699593
480 0.932760006189346
490 0.935359999537468
};
\addlegendentry{$k=20$}
\addplot [semithick, color1]
table {%
60 0.790319991111755
70 0.804559987783432
80 0.815760001540184
90 0.822120004892349
100 0.831039997935295
110 0.844039979577065
120 0.853360000252724
130 0.860960000753403
140 0.867400002479553
150 0.876959997415543
160 0.881159994006157
170 0.887559992074966
180 0.891079992055893
190 0.895119991898537
200 0.895839983224869
210 0.901199993491173
220 0.907559990882874
230 0.910960003733635
240 0.913679978251457
250 0.9175999969244
260 0.918400004506111
270 0.922319996356964
280 0.925079998373985
290 0.929879987239838
300 0.93128000497818
310 0.930439990758896
320 0.935440003871918
330 0.933560007810593
340 0.935319992899895
350 0.937080007791519
360 0.940359991788864
370 0.941839995980263
380 0.944680005311966
390 0.941520005464554
400 0.944439995288849
410 0.946480000019074
420 0.945920011401176
430 0.945919996500015
440 0.947919988632202
450 0.949679979681969
460 0.947200009226799
470 0.949000003933907
480 0.949359998106956
490 0.950680011510849
};
\addlegendentry{$k=40$}
\addplot [semithick, color2]
table {%
60 0.797719991207123
70 0.813119992613792
80 0.823359996080399
90 0.834159994125366
100 0.849639987945557
110 0.862319988012314
120 0.872359994053841
130 0.88071998655796
140 0.884959998726845
150 0.891719990968704
160 0.89755999147892
170 0.89959999024868
180 0.908959975838661
190 0.913599997758865
200 0.916639986634254
210 0.923280003666878
220 0.926759991049767
230 0.929120007157326
240 0.928400015830994
250 0.933680009841919
260 0.935799995064735
270 0.937999993562698
280 0.940320003032684
290 0.941639995574951
300 0.943559995293617
310 0.944519996643066
320 0.942039993405342
330 0.947319999337196
340 0.949119997024536
350 0.946359980106354
360 0.947999998927116
370 0.947959995269775
380 0.951080000400543
390 0.952920001745224
400 0.950999999046326
410 0.952840003371239
420 0.952040001749992
430 0.951800006628037
440 0.951800006628037
450 0.955359995365143
460 0.953799986839294
470 0.952799993753433
480 0.956279993057251
490 0.956080007553101
};
\addlegendentry{$k=60$}
\addplot [semithick, color3]
table {%
60 0.803359985351562
70 0.815199998021126
80 0.825599986314774
90 0.840480002760887
100 0.857839995622635
110 0.867399999499321
120 0.878199964761734
130 0.88764001429081
140 0.891759991645813
150 0.901839992403984
160 0.906440007686615
170 0.912800002098084
180 0.917840006947517
190 0.924080014228821
200 0.928760001063347
210 0.933440008759499
220 0.938239991664886
230 0.940719982981682
240 0.94083998799324
250 0.943079981207848
260 0.944479984045029
270 0.948999997973442
280 0.951599997282028
290 0.945400002598763
300 0.95063998401165
310 0.950400003790855
320 0.952920001745224
330 0.951719999313354
340 0.952799993753433
350 0.955240023136139
360 0.954639983177185
370 0.953759986162186
380 0.955759996175766
390 0.954760003089905
400 0.954599997401237
410 0.953919991850853
420 0.954000002145767
430 0.956359994411468
440 0.956839996576309
450 0.956560006737709
460 0.958079999685287
470 0.958080017566681
480 0.957280001044273
490 0.957160004973412
};
\addlegendentry{$k=80$}
\addplot [semithick, color4]
table {%
60 0.80443999171257
70 0.816760009527206
80 0.830879989266396
90 0.850359997153282
100 0.862840005755425
110 0.875279998779297
120 0.882959994673729
130 0.892560005187988
140 0.899359992146492
150 0.907839998602867
160 0.910239994525909
170 0.920680004358292
180 0.923759996891022
190 0.928239986300468
200 0.931719988584518
210 0.937520009279251
220 0.937159997224808
230 0.942760011553764
240 0.945200008153915
250 0.949480003118515
260 0.950480005145073
270 0.949920004606247
280 0.951880005002022
290 0.949720001220703
300 0.950560000538826
310 0.955000007152557
320 0.953279989957809
330 0.955439999699593
340 0.954439994692802
350 0.957080006599426
360 0.953680008649826
370 0.955759999155998
380 0.956880006194115
390 0.955199986696243
400 0.95495999455452
410 0.959000006318092
420 0.958479988574982
430 0.958200001716614
440 0.959040006995201
450 0.957720005512238
460 0.95984001159668
470 0.960080003738403
480 0.959600013494492
490 0.957559984922409
};
\addlegendentry{$k=100$}
\addplot [dashed, black]
table {%
60 0.806919991970062
70 0.819919982552528
80 0.835479989647865
90 0.853880003094673
100 0.867759999632835
110 0.878759998083115
120 0.887520003318787
130 0.897239983081818
140 0.907840013504028
150 0.912119990587234
160 0.915960010886192
170 0.919399988651276
180 0.926239988207817
190 0.927200019359589
200 0.928000009059906
210 0.932999983429909
220 0.935119986534119
230 0.934839999675751
240 0.935239985585213
250 0.93792000412941
260 0.938479986786842
270 0.938479998707771
280 0.940479999780655
290 0.940239998698235
300 0.941440004110336
310 0.941679999232292
320 0.941799992322922
330 0.941719996929169
340 0.94472000002861
350 0.942440012097359
360 0.94520001411438
370 0.943720003962517
380 0.9427600055933
390 0.9457200050354
400 0.947040024399757
410 0.947400006651878
420 0.946920001506805
430 0.945960006117821
440 0.948400005698204
450 0.949400001764298
460 0.952240008115768
470 0.948880016803741
480 0.951319998502731
490 0.951920014619827
};
\addlegendentry{$k=120$}
\end{axis}

\end{tikzpicture}


==> preambule/autres_packages.tex <==
\usepackage{biblatex} % for bibliography
\addbibresource{biblio.bib}
\usepackage{url}            % Pour citer les adresses web
\usepackage[T1]{fontenc}    % Encodage des accents
\usepackage[utf8]{inputenc} % Lui aussi

\usepackage{numprint}       % Histoire que les chiffres soient bien

\usepackage{amsmath}        % La base pour les maths
\usepackage{mathrsfs}       % Quelques symboles supplémentaires
\usepackage{amssymb}        % encore des symboles.
\usepackage{amsfonts}       % Des fontes, eg pour \mathbb.
\usepackage{stmaryrd}
\usepackage{adjustbox}

\usepackage{cancel}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{mathdots}
\usepackage{colortbl}

%\usepackage[svgnames]{xcolor} % De la couleur

%%% Si jamais vous voulez changer de police: décommentez les trois 
%\usepackage{tgpagella}
%\usepackage{tgadventor}
%\usepackage{inconsolata}

%%% Pour L'utilisation de Python
\usepackage{minted}
\usemintedstyle{friendly}

\usepackage{graphicx} % inclusion des graphiques
\usepackage{wrapfig}  % Dessins dans le texte.
\usepackage{changepage}
\input{tikz_schemas/preambule}
\usepackage{comment}
\usepackage{tikz}     % Un package pour les dessins (utilisé pour l'environnement {code})
\usepackage[framemethod=TikZ]{mdframed}


==> preambule/macros.tex <==
% Ce fichier contient toutes les macros que vous pouvez avoir envie de définir 
% si vous les utilisez plusieurs fois dans le document.

\PassOptionsToPackage{svgnames}{color}


% Un environnement pour bien présenter le code informatique
\newenvironment{code}{%
\begin{mdframed}[linecolor=green,innerrightmargin=30pt,innerleftmargin=30pt,
backgroundcolor=black!5,
skipabove=10pt,skipbelow=10pt,roundcorner=5pt,
splitbottomskip=6pt,splittopskip=12pt]
}{%
\end{mdframed}
}

% Un raccourci pour composer les unités correctement (en droit)
% Exemple: $v = 10\U{m.s^{-1}}$
\newcommand{\U}[1]{~\mathrm{#1}}

% Les guillemets \ofg{par exemple}
\newcommand{\ofg}[1]{\og{}#1\fg{}}
\DeclareMathOperator*{\argmin}{arg\,min}
% Le d des dérivées doit être droit: \frac{\dd x}{\dd t}
\newcommand{\dd}{\text{d}}

% La dérivée temporelle, tellement courante en physique, avec les d droits
\newcommand{\ddt}[1]{\frac{\dd #1}{\dd t}}

% Des parenthèses, crochets et accolades qui s'adaptent automatiquement à la 
% taille de ce qu'il y a dedans
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\pac}[1]{\left[#1\right]}
\newcommand{\paa}[1]{\left\{#1\right\}}

% Un raccourci pour écrire une constante
\newcommand{\cte}{\text{C}^{\text{te}}}

% Pour faire des indices en mode texte (comme les énergie potentielles)
\newcommand{\e}[1]{_{\text{#1}}}

% Le produit vectoriel a un nom bizarre:
\newcommand{\vectoriel}{\wedge}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\indep}{\perp \!\!\! \perp}
% To make images take the whole slide
\newcommand\Wider[2][5em]{%
\makebox[\linewidth][c]{%
  \begin{minipage}{\dimexpr\textwidth+#1\relax}
  \raggedright#2
  \end{minipage}%
  }%
}

==> preambule/special_beamer.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Beamer Presentation
% LaTeX Template
% Version 1.0 (10/11/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND THEMES
%----------------------------------------------------------------------------------------




\mode<presentation> {

% The Beamer class comes with a number of default slide themes
% which change the colors and layouts of slides. Below this is a list
% of all the themes, uncomment each in turn to see what they look like.

%\usetheme{default}
%\usetheme{AnnArbor}
%\usetheme{Antibes}
%\usetheme{Bergen}
%\usetheme{Berkeley}
%\usetheme{Berlin}
%\usetheme{Boadilla}
%\usetheme{CambridgeUS}
%\usetheme{Copenhagen}
%\usetheme{Darmstadt}
%\usetheme{Dresden}
%\usetheme{Frankfurt}
%\usetheme{Goettingen}
%\usetheme{Hannover}
%\usetheme{Ilmenau}
%\usetheme{JuanLesPins}
%\usetheme{Luebeck}
%\usetheme{Madrid}		
%\usetheme{Malmoe}
%\usetheme{Marburg}
%\usetheme{Montpellier}
%\usetheme{PaloAlto}
%\usetheme{Pittsburgh}
%\usetheme{Rochester}
%\usetheme{Singapore}
%\usetheme{Szeged}
\usetheme{Warsaw}

% As well as themes, the Beamer class has a number of color themes
% for any slide theme. Uncomment each of these in turn to see how it
% changes the colors of your current slide theme.

%\usecolortheme{albatross}
%\usecolortheme{beaver}
%\usecolortheme{beetle}
%\usecolortheme{crane}
%\usecolortheme{dolphin}
%\usecolortheme{dove}
%\usecolortheme{fly}
%\usecolortheme{lily}
%\usecolortheme{orchid}
%\usecolortheme{rose}
%\usecolortheme{seagull}
%\usecolortheme{seahorse}
\usecolortheme{whale}
%\usecolortheme{wolverine}

%\setbeamertemplate{footline} % To remove the footer line in all slides uncomment this line
%\setbeamertemplate{footline}[frame number] % To replace the footer line in all slides with a simple slide count uncomment this line

%\setbeamertemplate{navigation symbols}{} % To remove the navigation symbols from the bottom of all slides uncomment this line

\setbeamercovered{transparent} % Fait apparaître les animations en grisé (utile pour la conception, mais peut être commenté lors de la remise du document final)
\setbeamertemplate{bibliography item}{\insertbiblabel}

% Pour utiliser une police à empattements partout
\usefonttheme{serif}

% Pour rajouter la numérotation des frames dans les pieds de page
\newcommand*\oldmacro{}%
\let\oldmacro\insertshorttitle%
\renewcommand*\insertshorttitle{%
  \oldmacro\hfill%
  \insertframenumber\,/\,\inserttotalframenumber}

}

\usepackage{graphicx} % Allows including images
\usepackage{booktabs} % Allows the use of \toprule, \midrule and \bottomrule in tables



==> sections/abstract.tex <==
% !TEX root = ../main.tex

\begin{abstract}
	Deep multi-task methods, where several tasks are learned within a single network, have recently attracted increasing attention. Burning point of this attention is their capacity to capture inter-task relationships. Current approaches either only rely on weight sharing, or add explicit dependency modelling by decomposing the task joint distribution using Bayes chain rule. If the latter strategy yields  comprehensive inter-task relationships modelling, it requires imposing an arbitrary order into an unordered task set. Most importantly, this sequence ordering choice has been identified as a critical source of performance variations. In this paper, we present Multi-Order Network (MONET), a multi-task learning method with joint task order optimization. MONET uses a differentiable order selection based on soft order modelling inside Birkhoff’s polytope to jointly learn task-wise recurrent modules with their optimal chaining order. Furthermore, we introduce warm up and order dropout to enhance order selection by encouraging order exploration. Experimentally, we first verify MONET capacity to retrieve the optimal order in a toy environment. Second, we use an attribute detection scenario to show that MONET outperforms existing multi-task baselines on a wide range of dependency settings.  Finally, we demonstrate that MONET significantly extends state-of-the-art performance in Facial Action Unit detection.

%Deep multi-task methods, where several tasks are learned within a single network, have attracted increasing attention in the past few years. Burning point of this attention is their capacity to capture statistical inter-task relationships. To do so, current approaches either only rely on weight sharing, or add explicit dependency modelling by decomposing the task joint distribution using Bayes chain rule. If the latter strategy yields comprehensive inter-task relationships modelling, it requires imposing an arbitrary sequence structure into an a priori unordered tasks set. This sequence ordering choice has been identified as a critical source of variations in modelization performances. In this paper, we present our Multi-Order Network (MONET), a multi-task sequential ordering optimization method for binary classification. Architecturally, MONET is composed of a recurrent module for each task. Those modules are learned jointly with their optimal chaining order using a convex combination based order selection mechanism. Furthermore, MONET leverages an order dropout strategy that improves modules generalizability by forcing them to explore several orders of prediction. Experimentally, we first validate MONET capacity to retrieve the optimal order in a controlled toy environment. Second, we show that MONET consistently outperforms several existing baselines in multiple real-world scenario such as Attribute detection and Facial Action Unit (AU). On the latter, we further demonstrate that MONET extends state-of-the-art performances. 

%By training modules to predict tasks in multiple orders, MONET improves their generalizabilisation capacity. To further enhance this regularization, we introduce a drop-out like strategy that refines order selection to encourage order space exploration.
\end{abstract}




==> sections/conclusion.tex <==
% !TEX root = ../main.tex
In this paper, we introduced MONET, a multi-order network for joint task order and prediction modelling in deep multi-task learning. MONET leverages a differentiable order selection mechanism based on soft order modelling inside Birkhoff's polytope, as well as task-wise recurrent cell sharing for concurrent multi-order prediction learning. Furthermore, we propose an order dropout strategy that enhances order selection by preventing order overfitting.

Similar to MRNN, MONET models the set of tasks to predict as an ordered sequence. The toy dataset exemplifies a situation where this sequential modelling is optimal in a given order. In this controlled scenario, we proved that MONET converges towards the correct order and significantly outperforms its random order selection counterparts along with other existing multi-task baselines.

In general learning problems, we do not know whether task sequential modelling is beneficial compared to parallel prediction, nor, \textit{a fortiori}, if \textit{order} matters. In other words, we have no \textit{a priori} information on whether MONET modelisation is well-adapted or not to a given situation. Yet, we experimentally demonstrate that MONET display competitive performance on a wide variety of task relationship settings: applied to facial attribute detection (CelebA), MONET performs at least as well as the best multi-task baseline on each 5 attributes subset. Based on this empirical evidence, we argue that MONET is an all-around better multi-task method and could therefore constitute a valid architectural choice for many multi-task learning problems.

Furthermore, MONET surpasses state-of-the-art in AU detection (BP4D and DISFA), where tasks are known to display strong dependencies. It consequently paves the way toward better face related computational emotion description. In fact, we believe that extending MONET to other families of tasks (eg: categorical classification, regression) could help improve multi-task learning performance and in particular affective computing methods. Indeed, it would unlock better joint learning of multiple related face analysis tasks such as AU detection (binary classification), pose estimation (regression), identity recognition (categorical classification), arousal/valence regression, facial expression detection (categorical classification) and could enhance affective computing performance altogether.

Finally, the proposed work still suffers from certain limitations. The most important is the scalability to a large number of tasks. Indeed, the number of permutations for soft order modelling increases as the factorial of the number of tasks, and the number of recurrent cells in the architecture grows linearly with the number of tasks. A first intuition to reduce both the number of permutations and the number of used cells would be to partition the task space into blocks of conditionally independent tasks. Then we could use a recurrent cell by blocks of task and learn the best block order in a MONET-like fashion. However, this strategy comes with the problem of choosing which tasks should be grouped together in blocks. Grouping heuristics will be explored in future works.



==> sections/experiment.tex <==
% !TEX root = ../main.tex


\subsection{Datasets}


\textbf{Toy Dataset} For method empirical validation, we designed a 2-dimensional multi-task binary classification toy dataset represented in Figure \ref{fig:toy_distribution}. For $T$ tasks, it uses the  following laws for input and labels: 
\begin{equation}
\begin{aligned}
	\mathbf{X} &\sim \mathcal{U}([-1; 1]^{2}),\\
	\forall t\in [1, T] : Y_{T}^{(t)} &= \mathbf{1}_{\bigcup_{i=1}^{2^{t}}[b_{2i}^{(t)}, b_{2i + 1}^{(t)}]}(X^{(1)}),
\end{aligned}
\label{eq:toygen}
\end{equation}
where $b_{i}^{(t)} = -1 + \frac{i-1}{2^{t}}$. In short, $[-1; 1]^{2}$ is vertically split in a recurrent way. This dataset has a natural order in which the tasks are easier to solve: for $t\in [1, T]$, conditioning task $t+1$ by the $t$ first tasks results transforms it into an easy-to-solve classification problem with a single linear boundary. Conversely, conditioning task $t+1$ by the result of upcoming tasks in coordinate order do not simplify its complexity as a classification problem, it remains a $2^{t} - 1$ linear boundary problem . %Conditionally to $\mathbf{X}$, \gt{toy tasks are mutually independant. It shows that there is no obvious connection between task statistical dependencies and the order in which they should be processed (see supplementary)}.
We generate 500, 250 and 250 examples for the train, val and test partitions, respectively. Those sizes are deliberately small to challenge networks modelization performance.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/toy/toy_figure.png}
\caption{Distribution of $2000$ examples sampled from our toy dataset with $T=2$. Given task $1$, i.e given the left-right positioning of the sample w.r.t to the black dashed boundary, task $2$ is simplified into a single linear boundary learning problem represented by red boundaries.%For example, provided that a sample lies on the left side of the black boundary, task 2 is simplified into deciding weither it lies left or right of the left red boundary.
\label{fig:toy_distribution}} 
\end{figure}


\textbf{CelebA} is a widely used database in multi-task learning, composed of $\approx 200k$ celebrity images annotated with 40 different facial attributes. For performance evaluation, we measure accuracy score using the classic train ($\approx 160k$ images), valid ($\approx 20k$ images) and test ($\approx 20k$ images) partitions for 5 different subsets of 5 attributes each. Those subsets were chosen to test MONET behaviour in different dependency settings: 
\begin{itemize}
    \item \textit{gender}: with moustache, beard, lipstick, heavy makeup and sex detection. Those attributes display statistical dependencies. For example a beard often implies a moustache.
    \item \textit{accessory}: with earrings, eyeglasses, necklaces and neckties detection.
    \item \textit{beauty}: with arched eyebrows, attractiveness , high cheekbones, rosy cheeks, and oval faces detection.
    \item \textit{haircut}: with baldness, black, blond, brown and gray hair detection. Those attributes are mutually exclusive.
    \item \textit{miscellaneous}: with 5 o'clock shadow, pointy nose, mouth slighlty open, oval face, and weither the subject is young or not. Those attributes are independant \textit{a priori}.
\end{itemize}
Both \textit{accessory} and \textit{beauty} were choosen for their lack of clear a priori on the type of dependencies that bind the tasks together.

\textbf{BP4D} is a dataset for facial action unit detection. It is composed of approximately $140k$ images featuring $41$ people ($23$ female, $18$ male) with different ethnicities. Each image is annotated with the presence of $12$ AU. For performance evaluation, we follow related work strategy that is to report F1-Score on all $12$ AUs using a subject exclusive 3-fold cross-validation with publicly available fold repartition from \cite{shao2018deep} and \cite{shao2020jaa}.

\textbf{DISFA} is another dataset for facial action unit detection. It contains 27 videos for $\approx 100k$ face images. Those images were collected from $27$ participants and annotated with $12$ AUs. Originally, each AU label is an intensity score ranging from $0$ to $5.$. In detection, labels with an intensity score higher than 2 are considered positive \cite{zhao2016deep}. Similarly to BP4D, the performance evaluation protocol consists in measuring the F1-Score for $8$ AUs using a subject exclusive 3-fold cross validation.


%MONET parameters set cardinality grows linearly with the number of task, therefore we cannot afford training on the 40 attributes simultaneously. Consequently, we reduce the scope of our CelebA performance study to 5 subsets of 5 attributes each, covering at total of 24 attributes. Attributes and subsets are detailed in table \ref{tab:celeba_results}.  %We clearly identify the lack of scalability with the number of task as the main limitation of our method. We will discuss it further in the future works section.


\subsection{Implementation Details}
In our experiments, we compare MONET with several multi-task baselines, each using a shared encoder and a number of prediction heads. For VMN-Common (VMNC), the prediction head consists in two dense $\rightarrow$ BN $\rightarrow$ ReLU applications followed by another dense $\rightarrow$ sigmoid layer with $T$ outputs. VMN-Separate (VMNS) uses $T$ prediction heads, each with the same structure, except the last layer is of size $1$. Finally, MRNN uses a single Gated Recurrent Unit (GRU) cell which sequentially predicts the $T$ tasks. Task order is randomly sampled for each MRNN experiment.

\textbf{Toy Experiments: } The shared encoder consists of four dense layers with $64$ units and ReLU activation. Prediction heads for both VMNC and VMNS consist in dense layers with $64$ units. Both MRNN and MONET employ GRU cells with $64$ units and $L=20$ orders. All networks are trained by applying 500 epochs with Adam~\cite{adam}, batch size $64$ with an exponentially decaying base learning rate $5e-4$ and $\beta=0.99$.
MONET order selector is trained with Adam with learning rate $0.005$. Other MONET related parameters (dropout $k$, warmup $n$) are determined by hyperparameter tuning on a dedicated validation dataset.

\textbf{Face Attributes:} For CelebA we make use of an Inception resnet v1 encoder pretrained on VGGFace2 \cite{cao2018vggface2} along with dense layers with $64$ units as prediction heads for VMNC and VMNS. Both MRNN and MONET use GRU cells with $64$ units and $L=20$ orders. Networks are trained with $30$ epochs using AdamW~\cite{adamw} with learning rate/weight decay set to $0.0005$ and exponential decay ($\beta=0.96$). For MONET hyperparameters, we use $M=5!=120$ permutations and order dropout $k=32$.

\textbf{Facial Action Unit Detection : }
\begin{comment}
Action Units are relatively short events. Therefore video-based datasets such as DISFA and BP4D display a serious data imbalance problem (\cite{shao2020jaa}) that comes with two main obstacles that act as a barrier to successful learning:

\gt{First, for each action units, there are only few positive examples. We adapt our architecture to this imbalance, using the method proposed in \cite{lin2017focal} that is to initialize the last bias $b^{(t)}$ of the module that predicts the $t$-th AU so that $S(b^{(t)}) = f^{(t)}$, i.e:
\begin{equation}
    b^{(t)} = \log \frac{f^{(t)}}{1 - f^{(t)}}
\end{equation}
where $f^{(t)}$ is the frequency of the $t$-th AU in the training set.}

Second, the number of positive examples vary between the different AU. To take this imbalance into accounts we make use of the same method as in \cite{shao2020jaa} and weight the loss associated to each AU with its inverse occurence. This way, the AU with low frequencies w.r.t the others are not left away in the training process. For a given permutation $\sigma_{m}$, the associated element wise loss becomes :
\begin{equation}
    \mathcal{L}^{\sigma_m}_{i}(\theta) = \sum_{t=1}^{T} w^{\sigma_m(t)} BCE(y^{\sigma_m(t)}_{i}, p_{i, m}^{(t)}), 
\end{equation}
where $w^{(t)} = \frac{1/f^{(t)}}{\sum_{i=1}^{T} (1 / f^{(i)})}$.

\gt{Finally, We further adapt to the AU evaluation protocol that measure F1 score by adding a Dice score contribution (\cite{shao2020jaa, jacob2021facial}) to the final loss:
\begin{equation}
    Dice^{\sigma_m}_i(\theta) = \sum_{t=1}^{T} w^{\sigma_m(t)} (1 - \frac{2 y_{i}^{\sigma_m(t)} p_{i, m}^{(t)} + \epsilon}{(y_{i}^{\sigma_m(t)})^{2} + (p_{i, m}^{(t)})^{2} + \epsilon}),
\end{equation}
where $\epsilon = 1$ is a smoothing term (\cite{shao2020jaa}).
All in all the final loss that we optimize is : 
\begin{equation}
    \mathcal{L}_{tot}(\theta) = \sum_{i=1}^{N}\sum_{m=1}^{M} \pi_m (\mathcal{L}_{i}^{\sigma_m}(\theta) + \lambda Dice^{\sigma_m}_i(\theta)),
\end{equation}}
\end{comment}
Action Units are relatively short events. Therefore video-based datasets such as DISFA and BP4D display a data imbalance problem \cite{shao2020jaa} that may act as a barrier to efficient learning. To circumvent this problem, we combine  biais initialization \cite{lin2017focal} and per AU loss weighting \cite{shao2020jaa}. To further adapt to the evaluation protocol that measure F1 score we include a Dice score contribution \cite{shao2020jaa, jacob2021facial} to the final loss.

For BP4D, we use an Inceptionv3 backbone pretrained on imagenet on top of which we put a MONET instance with $M=512$ and $k=128$. The order selection part of MONET is trained using Adam with warmup $n=5$ and constant learning rate $5e-3$ while the rest of the network uses AdamW optimizer with learning rate/weight decay set to $1e-4$ and exponential decay $\beta = 0.99$. Batchsize is set to $16$, number of epochs is $2$ and dice loss coefficient is $\lambda=0.5$.

For DISFA, we make use of the same encoder as for CelebA  and retrain with AdamW learning rate $5e-4$ with exponential decay $\beta = 0.96$, and batchsize $64$. All other parameters stay the same as for BP4D.





%In all experiments, we report the average performance over 5 runs.

%All performance results are reported as $\mu \pm \frac{\sigma}{\sqrt{n}}$ where $\mu$ and $\sigma$ are respectively the mean and standard deviation on $n=5$ runs.





\subsection{Toy experiments}




%\begin{figure}
    %\centering
    %\input{tikz_schemas/M_k_validation}
    %\caption{MONET performances comparaison for toy dataset with $T=5$ between: (in red) dropout less version (k=M) for different values of $M$  and (in green) dropout version with M=T! and different values of $k$. Dashed and full black lines are respectively the random order selection baseline and the oracle mean performances. Means and standard deviations are computed on 10 runs.}
    %\label{fig:k_beats_M}
%\end{figure}

%\begin{table*}
%\centering
%    \caption{Comparison of MONET for different numbers of tasks $T$ and values of hyperparameters $M$ (number of orders) and $k$ (for order dropout). For nearly every run, MONET manages to find the correct order $\mathbf{I}_{T}$ and significantly outperforms the random order, approaching the oracle predictor with correct order.}
%    \vspace{0.1cm}
%    \label{tab:toy_order}
%    \input{tables/toy_order_export.tex}
%\end{table*}


\begin{figure}
\centering
    \caption{Performance of MONET trained with a single order $\sigma$ $(M=1, k=1)$ as a fonction of the frobenius distance between $\sigma$ and the identity order. Accuracy scores are averaged over 10 runs. \label{fig:order_matter}}
    \includegraphics[width=\linewidth]{figures/toy/ordermatter.pdf}
\end{figure}

Figure \ref{fig:order_matter} shows the performance of MONET trained with a single, imposed order $\sigma$ on the toy dataset with $T=3,4,5$. For all considered $T$, MONET reaches its best performance when $\sigma$ verifies $\|\mathbf{M}_{\sigma} - \mathbf{I}_{T}\|_{F}^{2} = 0$, which only occurs when the imposed order $\sigma$ is the identity order. Thus, the identity order is the optimal order in the toy experiment.

Furthermore, we observe a significant decrease in performance as the imposed order $\sigma$ moves away (\textit{i.e.} as expressed by the frobenius norm of the difference) from the identity order. More precisely, the further the chosen $\sigma$ is from the identity, the lower the accuracy of the network accross the $T$ tasks. Therefore, \textit{order matters} in the toy settings and the best performing orders are the identity order and the orders that are close to it.

\begin{table}
\centering
    \caption{Comparison of different order selection mechanism for $T = 5$ and $M = 120$. Performance are averaged over 10 runs.}
    \vspace{0.1cm}
    \label{tab:ablation_study}
    \input{tables/ablation_study.tex}
\end{table}

Table \ref{tab:ablation_study} displays the performance of MONET with different order selection mechanism versions. It reports mean accuracy averaged on 10 runs along with the number of times MONET selected the identity order (correct order in this setting) over these runs. As mentioned in the previous paragraph, those two quantities depend from one another because selecting the correct order results in higher performance. 

The worst performing method, that we called Hard Selection is an implementation of \cite{vinyals2015order} order selection mechanism. It uses an exploration phase similar to our warm up and then samples a single order using a distribution in which each order has a probability that is proportional to its performance (measured during exploration). Table \ref{tab:ablation_study} shows that this order selection mechanism perform poorly. In fact, we believe that such sampling strategy is sensitive to performance measurements noise and is therefore likely to result in a sub-optimal order. By smoothly learning its order selection coefficients all along the training phase, MONET gets a better estimation of each order performance and selects better orders.

Refining the order selection mechanism with warm up helps MONET to find better orders by providing an exploration phase to estimate each order performance before making a choice. However it doesn't prevent the order selection from snowballing, i.e to keep allocating weights to the first selected order. It explains that adding warm up to MONET only provides a tiny boost in performance.

\begin{figure*}
\centering
    \input{figures/toy/frob2Id.pgf}
    \caption{Evolution of the Frobenius distance between MONET soft order and the toy correct order for 20 MONET training with different values of $k$. \tac{Each line represent the soft order trajectory w.r.t the identity matrix for a different training of MONET.}\label{fig:frob2Id}}
\end{figure*}

Dropout on the other hand, short-circuit  the snowball effect by forcing the network to train on randomly selected orders: it allows MONET order selection mechanism to smoothly deviate from any previous choice of order. Indeed, figure \ref{fig:frob2Id}, shows that contrary to its standard version $(k=120, M=120)$, the dropout version of MONET $(k=100, M=120)$ is able to recover the correct order even if it started with a bad guess. Combined warmup and dropout provide MONET with an initial order guess that is likely to be good, and the ability to move away from this guess if needed. Those two ingredients result in better order selection which, in turn, implies better performance.




% Table \ref{tab:toy_order} draws a comparison between different versions of MONET, corresponding to different settings for hyperparameters $M$ (number of orders) and $k$ (number of kept orders with the proposed order dropout strategy), and with $T=4,5,6,7$ tasks. First of all, for $T=4,5$, there is a large gap in performance between MONET with random order $k/M=1/1$ and learned order ($k/M=24/24$ and $k/M=120/120$, for $T=4$ and $5$ tasks, respectively). This is likely due to the fact that, in the latter case, for both $T=4$ and $T=5$ tasks, MONET is able to successfully retrieve the correct order (corresponding to $\mathbf{I}_{T}$). In such a case, the network can correctly model the sequence of inter-task dependencies and learn adequate representation and prediction functions, hence superior performance.





% As such, it can be seen in Table \ref{tab:toy_order} that MONET with order dropout ($16/24$ and $80/120$ for $T=4$ and $5$ tasks respectively) matches the oracle performance for $T=4,5,6$ and significantly outperforms the random order baseline with larger number of tasks, e.g. $T=7$. As such, even for fairly high numbers of tasks $(T=6, 7)$, MONET using order dropout still manages to retrieve the correct order. Even when it doesn't manage to do so (1/5 when $T=7$) the order it finds still outperforms the random order selection baseline. The drop of performances between the oracle and the learned order version can be explained by the exploration time that MONET takes to find the correct order: intuitively, the smaller the $k/M$ ratio is, the more the exploration takes over the exploitation at train time.

%Figure \ref{fig:frob2Id} investigates the influence of $k$ on order exploration. It highlights that order selection without dropout ($k=120$) tend to snowball on early selected orders which explains its fast convergence as it quickly gets to fully exploit a single order. In contrast, the MONET version with $k=100$, takes more time to explore the order space and is able to switch order selection, even late in the training phase. In that extent, full single order exploitation occurs later in the training but exploits a better order than with $k=120$. This observation is consistent with the tendency observed in Figure \ref{fig:exploration_tradeoff}: $k=100$ takes more time to converge but reach higher performances at the end of the training.

\begin{table}
	\caption{Multi-task baselines comparaison on toy dataset with $T=5$ tasks. $^\dagger$: oracle predictor with correct order. \label{tab:toybaseline}}
	\vspace{0.1cm}
	\input{tables/toy_baselines.tex}
\end{table}



Finally, Table \ref{tab:toybaseline} shows relative performances of MONET w.r.t multi-task baselines.
% along with \cite{meyerson2017beyond} soft layer ordering (SLO) from which we drew MONET initial inspiration: 
MONET displays significantly better performances than all other considered methods, rivaling the oracle performance.

Eventually, we demonstrated in a controlled benchmark where an optimal task chaining order is known that (a) MONET was able to consistently retrieve said order, and (b) that thanks to its joint order selection mechanism and task-specific recurrent cell sharing architecture, backed by the proposed order dropout strategy, MONET was able to consistently outperform other multi-task baselines, getting closer to an oracle predictor using the optimal order. We now consider real-world applications with potentially more complex inter-task dependencies and less clear ordering patterns.


%competitive with MRNN provided with the correct order and outperforms its random selection counterparts. Furthermore, MONET and MRNN beat both VMN versions by a wide margin. Somehow this is surprising as in the toy generating equations (\ref{eq:toygen}), VMN inter-task conditional independance assumption holds. Actually, in the case of label conditional independance w.r.t the input, MRNN and MONET works as two different instanciations of VMN with specific task-wise weight sharing pattern. We believe that those specific weight sharing pattern are extremely well adapted to the toy data-structure and very hard to reproduce from scratch with a classic VMN.

\begin{comment}
 \\
The rise of the total number of orders with $T$, quickly make the training of MONET with all orders too computationally expensive. However, the last rows of table \ref{tab:toyorder} shows that MONET with low $k$ still manages to find the correct order and keeps outperforming the random order selection method for $T=6, 7$.

Table \ref{tab:toybaseline} shows relative performances of MONET w.r.t multi-task baselines: MONET displays competitive performances w.r.t MRNN provided with the correct order and outperforms its random selection counterparts. Furthermore, MONET and MRNN beat both VMN versions by a wide margin. Somehow this is surprising as in the toy generating equations (\ref{eq:toygen}), VMN inter-task conditional independence assumption hold. Actually, in the case of label conditional independence w.r.t the input, MRNN and MONET works as two different instanciations of VMN with specific task-wise weight sharing pattern. We believe that those specific weight sharing pattern are extremely well adapted to the toy data-structure and very hard to reproduce from scratch with a classic VMN.
\end{comment}


% Blabla sur exploration/exploitation à voir avec les résultats.

%In this section, we make use of our toy dataset to empirically validate our permutation selection mechanism. For that purpose, we train MONET on different instances of the toy dataset and track the evolution of MONET average permutation that we define as the $\pi$-weighted sum of its $M$ permutation matrices : 

%As we have mentionned before, the toy natural order is the coordinate order which associated permutation matrix is the identity matrix $\mathbf{I}_{T}$ To check if MONET finds the toy natural order, we measure the frobenius distance between $\bar{\mathbf{M}_\sigma}$ and $\mathbf{I}_{T}$ all along the training.\\
%The left part of figure (+ ref figure) reports the evol 

\subsection{Applications to face attribute detection}
%\subsubsection{Experiments on CelebA}
Table \ref{tab:celeba_results} draws a comparison between different multi-task methods for attribute detection on CelebA. On the one hand, there is no clear winner between the two VMN versions: for instance, VMNS performs better on the \textit{gender} and \textit{accessories} subsets while VMNC performs better on \textit{haircut} and \textit{misc.}. Those performance discrepancies may result in practical difficulties to find an all-around, well performing architecture, as echoed in \cite{misra2016cross}. Furthermore, MRNNs gets consistently outperformed by at least one of the VMN methods. In fact, we believe that MRNN recurrent cell sharing across tasks leads to early conflicts between task-associated gradients and prevents it from taking full advantage of its theoretically better inter-task relationship modelling. Additionally, random task order sampling may prevent MRNN from properly learning and hurt its predictive performance.  MONET, on the other hand, shows consistently better performances than both VMN as well as MRNN on every subset, due to both its task-wise modular weight sharing strategy and its order selection mechanism that, in turn, allows to correctly model inter-task dependencies.

\begin{table}[ht]
	\caption{Comparaison of MONET with multi-task baselines on several attributes subsets of CelebA. \label{tab:celeba_results}}
	\vspace{0.1cm}
	\centering
\input{tables/celeba_sota.tex}
\end{table}

Figure \ref{fig:celeba_matrices} depicts two soft-order matrices extracted at the end of MONET training on the \textit{gender} subset. First, those two matrices are very similar. Hence, MONET order selection mechanism is relatively stable across several networks and order selector initializations. Second, from a qualitative point of view, it appears that MONET first focuses on easier, specific tasks: it typically detects the attribute \textit{beard} (which intuitively are more visible) before \textit{mustache}, and \textit{lipstick} (which has a very characteristic color) earlier than \textit{heavy makeup} (which exhibit more variability). Then, in the light of the prediction of the aforementioned attributes, MONET concludes on the sex of the subject. To put it in a nutshell, MONET selects a suitable order for predicting the sequence of tasks, enhancing the final prediction accuracy.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/celeba/celeba_matrices.pdf}
    \caption{Two soft-order matrices extracted at the end of two different MONET training on CelebA \textit{gender} subset.     \label{fig:celeba_matrices}}
\end{figure}

\subsection{Applications to action unit detection}


\begin{table*}[ht]
	\caption{Comparaison of MONET with state-of-the-art deep learning based AU detection methods on BP4D \label{tab:bp4d_results}}
	\vspace{0.1cm}
	\input{tables/bp4d_sota.tex}
\end{table*}

\textbf{AU detection on BP4D:} Table \ref{tab:bp4d_results} draws a comparison between MONET and other state of the art deep approaches on the detection of 12 action units on BP4D database. Thanks to its order selection mechanism, MONET outperforms all the methods that explicitly models AU label dependencies such as DSIN or HMP-PS. More interestingly, it outperforms methods that use external information such as landmarks (EAC-NET, JAANET, PT-MT-ATsup-CC-E) or textual description of Action Units (SEV-NET). Finally, MONET performs better than PT-MT-ATsup-CC-E which leverages transformers in its architecture. Thus, despite the fact that there is considerable room for improvement, MONET outperforms existing approaches due to its ability to jointly model task order and prediction.

\begin{figure*}
\begin{adjustbox}{width=\linewidth}
\input{tikz_schemas/bp4d_facebook}
\end{adjustbox}
\caption{Samples of images from BP4D database with the AU groundtruth $(\mathbf{y})$ and MONET predictions $(\hat{\mathbf{y}})$. Each coordinate (represented by a square) represent a single AU (the order is AU1, AU2, AU4, AU6, AU7, AU10, AU12, AU14, AU15 AU17, AU23, AU25). A green square means that the AU is present in the image while a red square denotes its absence.\label{fig:bp4d_facebook}} 
\end{figure*}

Figure \ref{fig:bp4d_facebook} depicts images from BP4D along with their associated ground truth and MONET predictions. On the one hand, the left part (a, b, c) shows images where MONET predictions are fully accurate. It demonstrates that MONET is able to correctly classify both lowly expressive face (eg: (c, 3) and (c, 4)) and highly expressive ones (eg: (b, 2), (c, 2)). 

On the other hand, the right part (d, e, f) focuses on sources of error i.e on edge cases in which MONET predictions are inaccurate. First, annotations seems to be noisy. For example, (e, 4) is annotated with AU1 (the inner brow raiser) whereas the subject is clearly frowning. Similarly, image (d, 3) is annotated with AU17 (chin raiser) which can't occur while the mouth is open.

Second, MONET tends to include the subjects neutral face bias in its predictions. For example subject (f)'s face looks, to the human eye, biased towards AU2 (the outer brow raiser), meaning that his eyebrows are naturally raised when his face is neutral. MONET include this bias in its prediction and therefore predicts AU2  whereas it shouldn't because face bias are taken into account in FACS annotations.

Actually this particular source of error is fairly expected. Indeed, for a given expressive face image, MONET has no explicit information on the associated neutral face nor a fortiori on its bias. Consequently it cannot discriminate between an unbiased neutral face which display a particular AU (AU2 in (f) for example), and a neutral face that is biaised toward this particular AU.   

Finally, MONET is not fully accurate on faces that display very specific emotions. Typically (d, 3) seems to be yawning, (e, 4) displays fear/disgust and (f, 4) looks extremely puzzled. An explanation for MONET inaccurate predictions could be that BP4D do not provide enough examples for those specific facial expressions, that may involve low-probability AU combinations. In other words, the existing AU-annotated databases are not large enough to train a fully efficient classifier.


\textbf{AU detection on DISFA:} Table \ref{tab:disfa_results} compares the performance of  MONET with other state of the art approaches on DISFA. Similar to BP4D, MONET displays better performance than all other existing approaches. Therefore, MONET consistently outperform state of the art performance for facial action unit recognition.

\begin{table*}[ht]
	\caption{Comparaison of MONET with state-of-the-art deep learning based AU detection methods on DISFA \label{tab:disfa_results}}
	\vspace{0.1cm}
	\input{tables/disfa_sota.tex}
\end{table*}

Figure \ref{fig:disfa_matrices} shows MONET soft order evolution when training on DISFA. During the warm up phase (first 5 epochs), the soft order is the average of $512$ randomly sampled permutation matrices and is therefore close to uniform (all probabilities are close to $\frac{1}{T}$). At the end of the warm up, MONET starts learning the order selection coefficients. In particular, we observe that MONET tends to start by predicting AU1, 2, 4, 6, 9 which correspond to the upper part of the face (eyes and brows related action units) and then processes 12, 25 and 26 which are located in the lower part of the face (mostly the mouth). In fact we believe that tasks that use the same part of the image and more generally the same piece of information benefit from being processed close to each other.

This coarse intuition seems to be fairly verified at a more detailed scale as we also observe smaller blocks of consecutive tasks. For instance, AU25-26 basically focuses on mouth and jaw, and AU4-6 both have their regions of interest located around the eyes. As far as brow movements are concerned, it is worth noticing that AU4 is processed before AU1. An explanation could be that AU4 is easier to predict (mainly because it is less local as it often comes with nose and corner of the eye wrinkles). Therefore using AU4 prediction and learned dependencies to help predict AU1 is more beneficial than doing the opposite.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/disfa/disfa_matrices.pdf}
    \caption{Evolution of MONET soft order during 30 epochs of training on DISFA. For action unit $j$, the coefficient associated with timestep $i$ can be interpreted as the probability that action unit $j$ is processed at timestep $i$. \label{fig:disfa_matrices}}
\end{figure}

%Thanks to its order selection mechanism, MONET outperforms all the methods that explicitly models AU label dependencies such as DSIN or HMP-PS. More surprisingly it outperforms methods that use external information such as landmarks (EAC-NET, JAANET, PT-MT-ATsup-CC-E) or textual description of Action Units (SEV-NET). Finally it performs better than PT-MT-ATsup-CC-E which leverages transformers in its architecture. Thus, despite the fact that there is considerable room for improvement (landmark information incorporation and attention-based recurrent modeling), MONET outperforms existing approaches due to its ability to jointly model task order and prediction.}
% Table \ref{tab:disfa_results} shows a comparison between MONET and other state of the art deep approaches for facial action unit detection on DISFA database. Those performances are all the more interesting as methods such as EAC-NET \cite{li2018eac}, LP-NET \cite{niu2019local} or JAANET \cite{shao2020jaa} combines appearance features with additional geometric information based on facial landmarks, whereas MONET does not. 

% that takes two different aspects:}

%\gt{First, for a given AU there are drastically more negative examples than positives. Therefore a classifier trained with the usual binary crossentropy is likely to collapse into predicting zero for every examples. To circumvent this problem  we balance the positive/negative terms of each AU binary crossentropy using the inverse of the AU occurence frequencies.}

%\gt{Second, the number of positive examples vary a lot between AU. To take this imbalance into accounts we make use of the same method as in \cite{shao2020jaa} i.e to weight the loss associated to each AU with the ratio between the inverse frequency of this very AU and the sum of inverse frequencies of all AUs. This way, the AU with low frequencies w.r.t the others are not left away in the training process. All in all for a given permutation $\sigma_m$, the associated element_wise loss becomes :}

%Here again there is a large gap in performance between VMNC and VMNS. Furthermore, MRNN performance lies significantly lower than both VMN, likely due to the larger number of tasks, that makes it less likely to find a suitable order. Nevertheless, due to its order selection mechanism and the proposed order dropout strategy, MONET reaches significantly higher accuracies. Table \ref{tab:disfa_results} also shows a comparison between the proposed method and current state-of-the-art deep approaches on DISFA. Those performances are all the more interesting as methods such as EAC-NET \cite{li2018eac}, LP-NET \cite{niu2019local} or JAANET \cite{shao2020jaa} combines appearance features with additional geometric information based on facial landmarks, whereas MONET does not. Thus, despite the fact that there is considerable room for improvement, MONET outperforms existing approaches due to its ability to jointly model task order and prediction.

% Paragraphe sur les baselines



==> sections/introduction.tex <==
% !TEX root = ../main.tex


Deep multi-task learning methods have recently shown excellent results in diverse applicative fields including face analysis \cite{ranjan2017hyperface,zhang2014facial,lu2017fully}, image segmentation \cite{kendall2018multi} and natural language processing \cite{dong2015multi}. At the heart of those successes is the ability to capture inter-task relationships through weight sharing and explicit dependency modelling. The most widely adopted strategy \cite{ranjan2017hyperface, kokkinos2017ubernet} is to assume tasks conditional independence given the input. Such method uses a common encoder and predicts the different tasks using separate regressors in parallel (Figure \ref{fig:monet_overview}-(a)).

Concurrently, several works \cite{nam2017maximizing,liu2016recurrent} leveraged recurrent architectures to predict tasks in a sequential fashion (Figure \ref{fig:monet_overview}-(b)). The main benefit of such approach is that it enables better joint distribution modelization. In particular, it relaxes the conditional independence hypothese, hence taking into account inter-task relationships that do not depend on the input.

\begin{figure}
\vspace{-0.5cm}
	\resizebox{\columnwidth}{!}{
	\input{tikz_schemas/bigpicture_export.tex}}
	\caption{Overview of MONET along with existing multi-task methods. \tac{Modules (rounded rectangles) with the same color share weights.} (a) VMN models inter-task relationships through sharing encoder weights. (b) MRNN imposes an arbitrary task order. (c) MONET predicts the set of tasks in different orders using separate recurrent cells, one for each task. Those predictions are normalized to a common order (rounded arrows) so that they can be weighted by a convex combination to output the final prediction. By jointly learning the coefficients associated with each order along with the task-specific cells, MONET smoothly selects the best order of prediction and achieves superior performance.
	% achieves superior performances by jointly optimizing task order selection and predictions.
	}
	\label{fig:monet_overview}
	\vspace{-0.5cm}
\end{figure}

However, contrary to standard sequence processing, the set of tasks to predict has no natural order \textit{a priori}. Therefore, making task prediction sequential requires enforcing an arbitrary order into the set of tasks.
Crucially, recurrent networks performance have been proven sensitive to the order in which elements are predicted \cite{vinyals2015order}. Consequently, in the frame of multi-task learning using recurrent networks where predicted elements are tasks, the task prediction \textit{order matters}.

In this paper, we follow this sequential order optimization paradigm and introduce Multi-Order Network (MONET). MONET leverages permutation matrices to represent task orders. More precisely, it navigates between orders by learning a convex combination of permutation matrices (a soft order). In that extent MONET explores the convex hull of permutation matrices  (Birkhoff's polytope) to smoothly select the best order. Figure \ref{fig:monet_overview}-(c) illustrates MONET architecture for a 3-tasks problem. To summarize, the contributions of this work are the following:
% MONET explores several task orders by navigating Birkhoff's polytope of soft orders, and smoothly selects the best one.  \begin{comment}

\begin{itemize}
	\item We introduce MONET, a multi-task learning method with joint task order optimization and prediction. From an architectural standpoint, MONET uses soft order selection in Birkhoff's polytope as well as task-wise cell sharing to model task order and prediction in an end-to-end manner.
	\item From a learning standpoint, we introduce order dropout and warm up strategies that work hand in hand with the order selection to encourage modules to keep good predictive performances in several orders of prediction.
	%It consequently enhances order exploration and improves the modules generalization capacity.
	\item Experimentally, we demonstrate MONET capacity to retrieve the correct order on a carefully designed toy dataset. Then, we show that MONET outperforms several existing multi-task approaches on a wide range of attribute detection problems with diverse level of task dependency. Finally, we point out that MONET extends state-of-the-art performance in action unit detection which is a multi-task affective computing problem.
\end{itemize}

\begin{comment}
The rest of the paper is organized as follows: in Section \ref{sec:related} we review existing state-of-the-art approaches for action unit detection with an emphasis on multi-task approaches. Then, in Section \ref{sec:methodology} we describe the proposed Multi-Order Network (MONET) method. In Section \ref{sec:experiments} we thoroughly validate MONET, firstly by evaluating its capacity to retrieve the correct order on a toy dataset, Secondly by showing that it achieves state-of-the-art accuracy on real-world multi-tasks problems such as face attribute prediction and action unit detection. Lastly, in Section \ref{sec:conclusion} we provide conclusive remarks and discuss future works.
\end{comment}


% (rounded arrows in Figure (\ref{fig:monet_overview}))
%approaches that models all task dependencies through Bayes chain rule decomposition.   On the exhaustive modelling side of the line, (\cite{nam2017maximizing}) have tried arranging the set of tasks in an arbitrary order and used a RNN-like architecture to model the joint conditional of task given inputs. (vinyals) criticizes this arbitrary choice of order, showing that task ordering matters in predictive performances. In the light of this claim they proposed a strategy that, first measures the modelization performances of several orders, then selects the best order once and for all based on those measurement, and finally continues training with this order only. However modelization performances measurements are based noisy signals. Therefore once and for all selection based on those quantities comes with a risk of getting definitevely stuck with a sub-optimal order. \\
%In the light of this claim, we propose our Multi Order Network (MONET), a deep multi-task architecture that explores several possible task orderings and aims at selecting the best one. More precisely, MONET trains a predictor per task jointly with an order selection mechanism that smoothly learns the best way to chain those predictors. \\
%Experimentally, we first show MONET order selection mechanism empirical validity on a well-chosen toy dataset. Then we demonstrate that MONET achieves competitive performances on two large scale multi-label binary classification problems. Namely Facial Action Unit (AU) detection on DISFA and facial attribute detection on CelebA. 
      
%% Background



==> sections/related.tex <==
\subsection{Multi-Task Learning}
Deep multi-task learning methods is a subset of deep learning methods that aim at exploiting similarities between several tasks in order to improve individual task performance. To reach that goal, the most widely adopted method relies on implicit modelling of task dependencies using weight sharing. In a nutshell, it consists in splitting the model into parts that are shared across tasks and parts that are task specific.

Seminal work \cite{ranjan2017hyperface, zhang2014facial, wu2015deep, kokkinos2017ubernet}, adopted this weight sharing strategy by making use of a common encoder along with task specific regressors. The intuition behind this is that forcing the same learned features to predict several related task should encourage the encoder to produce more general representations and consequently improve generalization performances. However, one weakness of this method comes with deciding how far features should be shared. Indeed, it intuitively depends on task relatedness (the more related the tasks the further the sharing) which can be hard to determine. To tackle this issue, numerous approaches \cite{ruder2017overview, misra2016cross, gao2019nddr, LiuSY19} used adaptative architectures to jointly learn which layers should be shared between tasks, as well as the task prediction itself. This philosophy has also been used in modular approaches which consist in learning a set of trainable modules along with how they should be combined for each tasks. For instance, soft layer ordering \cite{meyerson2017beyond} consists in learn the best module combination for each task in a fully differentiable way. In the same vein, a select or skip policy \cite{sun2020adashare} was used to determine which module should be used for each task.  

 Weight sharing may help finding features that are useful for all tasks and therefore implicitly models input-related task conditional dependencies, though, it doesn't capture inter-task relationships that do not depend on input (e.g the prior that detection of a beard implies high probability that the subject also has a mustache). In order to model those dependencies, several approaches \cite{ruder2017overview, nam2017maximizing, bilen2016integrated} leveraged recurrent neural networks to decompose the task joint distribution into a product of conditional distributions using Bayes chain rule. Most importantly, the work in \cite{vinyals2015order} showed that \textit{order matters}, meaning that the order in which the chain rule is unrolled impacts the final joint estimate modelization performance. In the light of this observation it proposes a two-steps method: The first step consists in an exploration phase in which the performance of several orders are tested. At the end of this phase, a single order is fixed once and for all based on the exploration phase performance and predictions are computed using this order.

Our work lies in the continuity of the order optimization paradigm proposed in \cite{vinyals2015order} which aim at improving current Bayes chain rule based joint distribution estimation. However, we stand out from it by drawing inspiration in \cite{meyerson2017beyond} to: (a) Propose a soft order selection mechanism that navigates through Birkhoff's polytope, and (b) Propose a new task-wise modular recurrent architectural design. More precisely, MONET smooth selection contrasts with the once and for all choice of order in \cite{vinyals2015order} by keeping on learning several orders during all the training phase. We take full advantage of this by adding warm up and order dropout mechanisms that encourage modules to display good predictive performances for several orders of prediction. 

By optimizing the task order, MONET takes advantage of situations where \textit{order matters}. Furthermore, we believe that learning more than one task order all along the training improves MONET generalization capacity and thus predictive performance in more general multi-task settings where order do not necessarily matter.

\subsection{Action Unit Detection.}
The Facial Action Coding System (FACS) is a language that anatomically describes facial expressions using a dictionary of unitary muscular movements called Action Units (AU). Originally, it was designed by psychologists to provide unbiased facial emotion descriptions \cite{ekman1997face}. Consequently, automatic detection of such movements could help unlock better computational emotion analysis and improve face-based affective computing applications altogether (pain detection, emotion analysis, etc). From a machine learning point of view, AU detection consists in predicting the presence of each considered muscular activations. Therefore it is a multi-task problem in which each task corresponds to the prediction of a single AU. So far the research work have been gravitating around two specifities of the AU detection problem.

First, action units are local events meaning that the face zones in which they occur are relatively small and constrained. For instance AU1 (inner brow raiser) and AU2 (outer brow raiser) can only occur on the forehead. To tackle that challenge, prior work \cite{zhao2016deep} relaxed convolutional layers weight sharing constraint by introducing region-wise filters. The incentive is that using different filters on each region will result in a refined skin texture representation. However, the performance of such method is conditioned upon face alignment i.e upon weither or not specific face parts are always located in the same rectangular region. To circumvent this limitation several works \cite{li2017eac, shao2018deep, shao2020jaa} used facial key-points along with predefined attention maps to guide the extraction of AU-related features. More precisely, in  \cite{li2017eac}, predefined key-points were used to crop AU related zones while the works in \cite{li2017eac} and \cite{shao2019facial} used attention-like mechanisms based on fixed and jointly learned facial landmark predictors respectively.

Second, because of both social and physiological constraints, action units display strong dependencies between each other (eg: AU1 and AU2 often co-occurs while AU1 and AU4 are incompatible). From an intuitive point of view the exploitation of those dependencies is key to unlock better performance. Indeed, it could enable the use of easy-to-predict AU as a proxy to estimate the harder ones. For example, predicting first AU4 (brow lowerer) could help predict more subtle movements of the eyes such as AU1 or AU6 (cheek raiser). Several works focus on explicitly modeling those dependencies. In particular, backpropagation through a probabilistic graphical model (PGM) was adopted in \cite{Corneanu_2018_ECCV}, and an hybrid message passing strategy was used in \cite{song2021hybrid}. Others leveraged the local nature of AU to assume that label dependencies imply dependencies between local face zones. Attempts at capturing such spatial dependencies include attention map learning \cite{shao2019facial}, LSTM-based spatial pooling \cite{niu2019local} and more recently transformer-like architectures \cite{jacob2021facial}.

MONET stands on the line drawn by \cite{Corneanu_2018_ECCV} in the extent that it explicitly models AU labels dependencies. Slightly different from PGM backpropagation \cite{Corneanu_2018_ECCV}, it leverages recurrent cells to exploit AU relationships in a end to end fashion. More precisely, we draw inspiration from the general multi-task learning literature to devise an architecture that parallely learns the joint AU distribution in multiple orders and jointly select the best estimations. The main incentive behind this design is to find the orders in which each AU prediction best simplifies the learning of the following ones.

\begin{comment}
The rest of the paper is organized as follows: First, in Section \ref{sec:methodology} we describe existing multi-task baselines and introduce the proposed MONET framework for joint task order modelling and prediction. Then, in Section \ref{sec:experiment} we qualitatively and quantitatively validate MONET on a toy database as well as in real-world scenarios for attribute detection and facial action unit detection. In particular, we show that MONET consistently outperforms existing baselines and state-of-the-art approaches. Finally, in Section \ref{sec:conclusion} we discuss the limitations of MONET and provide conclusive remarks. \gt{ça je pense qu'on pourrait l'enlever et fill la place par une explication du titre.}
\end{comment}


==> tables/full_ablation_study.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Warm up & Dropout & Hard Selection & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Mean Accuracy & Finds $\mathbf{I}_{T}$ ? \\ 
%\hline
%2 & 1 & random & 1 & 2/5 & $100 $ & $98.7 $ & - & - & - & - & - & $99.3 $ \\
%2 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 2 & 5/5 & $100 $ & $98.9 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 1 & 0/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%\hline
%3 & 1 & random & 1 & 2/5 & $99.9 $ & $99.8 $ & $97.4 $ & - & - & - & - & $98.7 $ \\
%3 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100.0 $ & $99.2 $ & $97.0 $ & - & - & - & - & $98.6 $ \\
%3 & 6 & random & 6 & 5/5 & $100.0 $ & $99.2 $ & $97.2 $ & - & - & - & - & $98.8 $ \\
%3 & 6 & random & 4 & 5/5 & $100.0 $ & $99.1 $ & $97.2 $ & - & - & - & - & $98.7 $ \\
\hline
\ding{55} & \ding{55} & \checkmark & 99.4 & 95.2 & 70.8 & 55.9 & 49.7 & 74.2 & 0/10 \\
\ding{55} & \ding{55} & \ding{55} & 99.4 &	98.2 & 95.7	& 88.6	& 64.5 & 89.2 & 8/10 \\
\checkmark & \ding{55} & \ding{55} & 99.5 &	97.7 & 94.8	& 88.8	& 65.7 & 89.3& 9/10\\
\ding{55} & \checkmark & \ding{55} & \textbf{99.5} &  \textbf{98.8} & 95.4 & 89.8 & 65.4 & 89.8 & 10/10 \\  
\checkmark & \checkmark & \ding{55} & 99.4 & 98.3 & \textbf{95.8} & \textbf{90.0} & \textbf{68.2} & \textbf{90.1} & 10/10 \\  
\hline
\end{tabular}}


==> tables/full_celeba_sota.tex <==
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
% &\multicolumn{6}{|c|}{Celeba Gender}\\
% \hline \hline
 \footnotesize Gender & \footnotesize H. Makeup & \footnotesize Male & \footnotesize Mustache & \footnotesize No Beard & \footnotesize W Lipstick & Avg. \\
 \hline
 VMNC & $88.0 \pm 1.3$ & $95.8 \pm 1.0$ & $96.6 \pm 0.0$ & $95.4 \pm 0.1$ & $90.2 \pm 1.8$ & $93.2 \pm 0.6$ \\
 VMNS & $90.2 \pm 0.1$ & $97.0 \pm 0.0$ & $96.7 \pm 0.0$ & $95.5 \pm 0.1$ & $93.9 \pm 0.0$ & $94.6 \pm 0.0$ \\
 MRNN & $89.9 \pm 0.1$ & $96.9 \pm 0.1$ & $96.7 \pm 0.0$ & $95.6 \pm 0.1$ & $93.6 \pm 0.0$ & $94.5 \pm 0.0$ \\
 MONET & $90.5 \pm 0.0$ & $97.5 \pm 0.0$ & $96.8 \pm 0.0$ & $95.8 \pm 0.0$ & $93.9 \pm 0.0$ & $\mathbf{94.9 \pm 0.0}$ \\
 \hline
 \hline
\footnotesize Accessories & \footnotesize Eyeglasses & \footnotesize W Earrings &\footnotesize W Hat &\footnotesize W Necklace &\footnotesize W Necktie & Avg. \\
 \hline
 VMNC & $99.4 \pm 0.1$ & $88.5 \pm 0.5$ & $98.4 \pm 0.1$ & $86.8 \pm 0.1$ & $95.8 \pm 0.3$ & $93.8 \pm 0.2$\\
 VMNS & $99.5 \pm 0.0$ & $89.5 \pm 0.1$ & $98.6 \pm 0.0$ & $87.1 \pm 0.0$ & $96.7 \pm 0.0$ & $\mathbf{94.3 \pm 0.0}$ \\
 MRNN & $99.5 \pm 0.0$ & $89.6 \pm 0.1$ & $98.7 \pm 0.0$ & $87.1 \pm 0.0$ & $96.6 \pm 0.1$ & $\mathbf{94.3 \pm 0.0}$ \\
 MONET & $99.2 \pm 0.3$ & $89.9 \pm 0.1$ & $98.5 \pm 0.2$ & $87.3 \pm 0.0$ & $96.8 \pm 0.0$ & $\mathbf{94.3 \pm 0.1}$ 
 \hline
 \hline
\footnotesize Haircut &\footnotesize Bald &\footnotesize Black Hair &\footnotesize Blond Hair &\footnotesize Brown Hair &\footnotesize Gray Hair & Avg. \\
 \hline
 VMNC & $98.6 \pm 0.0$ & $88.3 \pm 0.3$ & $95.3 \pm 0.0$ & $88.0 \pm 0.2$ & $98.0 \pm 0.0$ & $93.6 \pm 0.1$\\
 VMNS & $98.6 \pm 0.0$ & $86.2 \pm 0.8$ & $95.2 \pm 0.0$ & $86.9 \pm 0.2$ & $97.9 \pm 0.0$ & $93.0 \pm 0.1$ \\
 MRNN & $98.6 \pm 0.0$ & $86.7 \pm 0.6$ & $95.2 \pm 0.0$ & $86.2 \pm 0.8$ & $97.8 \pm 0.0$ & $92.9 \pm 0.2$ \\
 MONET & $98.7 \pm 0.0$ & $88.3 \pm 0.4$ & $95.4 \pm 0.1$ & $88.0 \pm 0.3$ & $98.0 \pm 0.0$ & $\mathbf{93.7 \pm 0.1}$ \\
 \hline
 \hline
\footnotesize Beauty &\footnotesize A Eyebrows &\footnotesize Attractive &\footnotesize H ChBones &\footnotesize R Cheeks &\footnotesize Oval Face & Avg. \\
 \hline
 VMNC & $82.8 \pm 0.0$ & $81.1 \pm 0.1$ & $86.8 \pm 0.0$ & $94.2 \pm 0.1$ & $73.7 \pm 0.2$ & $83.7 \pm 0.0$ \\
 VMNS & $82.5 \pm 0.1$ & $81.0 \pm 0.1$ & $86.5 \pm 0.1$ & $94.4 \pm 0.0$ & $74.0 \pm 0.2$ & $83.7 \pm 0.1$ \\
 MRNN & $82.8 \pm 0.0$ & $80.6 \pm 0.3$ & $86.3 \pm 0.2$ & $94.6 \pm 0.0$ & $74.1 \pm 0.0$ & $83.7 \pm 0.0$ \\
 MONET & $82.8 \pm 0.1$ & $81.5 \pm 0.1$ & $86.9 \pm 0.1$ & $94.7 \pm 0.0$ & $74.4 \pm 0.1$ & $\mathbf{84.1 \pm 0.1}$ \\
 \hline
 \hline
\footnotesize Misc. &\footnotesize  5 Shadow &\footnotesize P Nose &\footnotesize M S Open &\footnotesize Oval Face &\footnotesize Young & Avg. \\
 \hline
 VMNC & $93.6 \pm 0.1$ & $76.6 \pm 0.1$ & $93.5 \pm 0.1$ & $74.2 \pm 0.0$ & $86.4 \pm 0.0$ & $84.9 \pm 0.0$ \\
 VMNS & $93.6 \pm 0.2$ & $76.7 \pm 0.2$ & $84.8 \pm 7.6$ & $74.1 \pm 0.1$ & $86.8 \pm 0.1$ & $83.2 \pm 1.5$ \\
 MRNN & $93.6 \pm 0.1$ & $76.1 \pm 0.5$ & $93.2 \pm 0.2$ & $73.6 \pm 0.4$ & $85.6 \pm 0.9$ & $84.4 \pm 0.2$ \\
 MONET & $94.2 \pm 0.0$ & $76.7 \pm 0.0$ & $93.6 \pm 0.1$ & $74.3 \pm 0.1$ & $87.0 \pm 0.1$ & $\mathbf{85.2 \pm 0.0}$ \\
 \hline
\end{tabular}
}


==> tables/order_matter.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
T & Rank & Order & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Mean Accuracy \\ 
%\hline
%2 & 1 & random & 1 & 2/5 & $100 $ & $98.7 $ & - & - & - & - & - & $99.3 $ \\
%2 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 2 & 5/5 & $100 $ & $98.9 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 1 & 0/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%\hline
%3 & 1 & random & 1 & 2/5 & $99.9 $ & $99.8 $ & $97.4 $ & - & - & - & - & $98.7 $ \\
%3 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100.0 $ & $99.2 $ & $97.0 $ & - & - & - & - & $98.6 $ \\
%3 & 6 & random & 6 & 5/5 & $100.0 $ & $99.2 $ & $97.2 $ & - & - & - & - & $98.8 $ \\
%3 & 6 & random & 4 & 5/5 & $100.0 $ & $99.1 $ & $97.2 $ & - & - & - & - & $98.7 $ \\
\hline
3 & 1 & [0, 1, 2] & 99.3 & 98.8 & 95.5 & - & - & 97.8 \\
  & 2 & [1, 2, 0] & 99.2 & 98.2 & 95.2 & - & - & 97.5 \\
  & 3 & [1, 0, 2] & 99.4 & 97.8 & 95.0 & - & - & 97.4 \\
  & 6 & [2, 0, 1] & 99.3 & 88.9 & 70.8 & - & - & 86.3 \\
  & * & random & 99.2 & 95.5 & 89.0 & - & - & 94.6  \\
\hline\hline
4 & 1 & [0, 1, 2, 3] & 99.7 & 98.6 & 95.8 & 91.5 & - & 96.5\\
  & 2 & [1, 2, 3, 0] & 99.4 & 98.6 & 95.8 & 92.0 & - & 96.5 \\
  & 3 & [1, 0, 2, 3] & 99.5 & 98.0 & 95.0 & 91.8 & - & 96.0 \\
  & 24 & [2, 3, 0, 1] & 99.4 & 90.4 & 69.9 & 57.7 & - & 79.4 \\
  & * & random & 99.4 & 94.0 & 84.1 & 73.6 & - & 87.8  \\
  
\hline\hline
5 & 1 & [0, 1, 2, 3, 4] & 99.6 & 98.6 & 96.1 & 92.1 & 80.6 & 93.4 \\
  & 2 & [1, 2, 0, 3, 4] & 99.4 & 98.2 & 95.0 & 92.0 & 81.2 & 93.1 \\
  & 3 & [1, 0, 2, 3, 4] & 99.5 & 97.1 & 94.3 & 91.1 & 81.8 & 92.7 \\
  & 120 & [2, 4, 3, 0, 1] & 98.9 & 91.1 & 67.4 & 56.4 & 49.4 & 72.6 \\
  & * & random & 99.3 & 93.9 & 78.2 & 65.4 & 51.9 & 77.8 \\
 \hline
\end{tabular}}


==> tables/toy_order.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|l|c|c|c|c|c|c|c|c|c|c|}
\hline
T & k/ M & order & Finds $\mathbf{I}_{T}$? & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Task 7 & Mean \\ 
%\hline
%2 & 1 & random & 1 & 2/5 & $100 $ & $98.7 $ & - & - & - & - & - & $99.3 $ \\
%2 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 2 & 5/5 & $100 $ & $98.9 $ & - & - & - & - & - & $99.4 $ \\
%2 & 2 & random & 1 & 0/5 & $100 $ & $98.8 $ & - & - & - & - & - & $99.4 $ \\
%\hline
%3 & 1 & random & 1 & 2/5 & $99.9 $ & $99.8 $ & $97.4 $ & - & - & - & - & $98.7 $ \\
%3 & 1 & $\mathbf{I}_{T}$ & 1 & 5/5 & $100.0 $ & $99.2 $ & $97.0 $ & - & - & - & - & $98.6 $ \\
%3 & 6 & random & 6 & 5/5 & $100.0 $ & $99.2 $ & $97.2 $ & - & - & - & - & $98.8 $ \\
%3 & 6 & random & 4 & 5/5 & $100.0 $ & $99.1 $ & $97.2 $ & - & - & - & - & $98.7 $ \\
\hline
4 & 1/1 & random & 0/5 & $99.9 $ & $97.4 $ & $92.3 $ & $82.1 $ & - & - & - & $92.9 $ \\
  & 24/24 & learned & 5/5 & $100.0 $ & $99.3 $ & $96.3 $ & $92.1 $ & - & - & - & $96.9 $ \\
 & 16/24 & learned & 5/5 & $100.0 $ & $99.2 $ & $97.5 $ & $94.7 $ & - & - & - & $97.8 $ \\
 \hline
\rowcolor{lightgray} Oracle & 1/1 & $\mathbf{I}_{T}$ & 5/5 & $100.0 $ & $99.5 $ & $97.4 $ & $94.0 $ & - & - & - & $97.7 $ \\
\hline\hline
5 & 1/1 & random & 0/5 & $99.9 $ & $96.6 $ & $88.4 $ & $72.9 $ & $63.4 $& - &-  & $ 84.2$ \\
 & 120/120 & learned & 5/5 & $100.0 $ & $99.3 $ & $97.1 $ & $94.1 $ & $88.8 $ & - & - & $95.8 $\\
 & 80/120 & learned  & 5/5 & $100.0 $ & $99.4 $ & $96.7 $ & $93.5 $ & $88.3 $ & - & - & $95.5 $\\
  \hline
\rowcolor{lightgray} Oracle & 1/1 & $\mathbf{I}_{T}$ & 5/5 & $100.0 $ & $99.5 $ & $97.7 $ & $94.2 $ & $90.1 $ & - & - & $96.3 $ \\
\hline\hline
6 & 1/1 & random & 0/5 & $99.9 $ & $97.5 $ & $91.2 $ & $70.6 $ & $58.2 $ & $56.4 $ & -  & $78.9 $ \\
 & 480/720 & learned & 5/5 & $100.0 $ & $99.2 $ & $97.4 $ & $94.1 $ & $90.0 $ & $79.1 $ & - & $93.3 $\\
 \hline
\rowcolor{lightgray} Oracle & 1/1 & $\mathbf{I}_{T}$ & 5/5 & $100.0 $ & $99.1 $ & $97.6 $ & $93.9 $ & $90.6 $ & $82.4 $  & - & $93.9 $ \\
\hline\hline
7 & 1/1 & random & 0/5 & $99.9 $ & $97.2 $ & $87.6 $ & $73.1 $ & $63.4 $ & $55.1  $ & $57.3 $ & $76.2 $ \\
 & 480/5040 & learned & 4/5 & $100.0 $ & $99.2 $ & $96.5 $ & $91.9 $ & $65.9 $ & $55.9 $ & $56.8 $ & $80.9 $ \\
\hline
\rowcolor{lightgray} Oracle & 1/1 & $\mathbf{I}_{T}$ & 5/5 & $100.0 $ & $99.1 $ & $97.3 $ & $94.4 $ & $90.3 $ & $84.4 $ & $67.9 $ & $90.5 $ \\
 \hline
\end{tabular}}

